Asymptotic Hodge Theory in String Compactifications and Integrable Systems

In this thesis we study the framework of asymptotic Hodge theory and its applications in both the string landscape and the landscape of 2d integrable field theories. We show how this mathematical framework allows for a general characterization of the asymptotic behaviour of physical couplings in low-energy effective theories coming from string theory, and apply this knowledge to investigate the finiteness and geometric structure of the string landscape landscape. At the same time, we find that the defining equations of variations of Hodge structure also arise in the context of certain integrable field theories, which opens the way to finding new classes of very general solutions to said models. Part I reviews the relevant aspects of type IIB / F-theory flux compactifications and the resulting landscape of 4d low-energy effective $\mathcal{N}=1$ supergravity theories. Part II provides an in-depth discussion on asymptotic Hodge theory, including detailed explanations on the nilpotent orbit theorem of Schmid, and the multi-variable Sl(2)-orbit theorem of Cattani, Kaplan, and Schmid. This part of the thesis also contains new results regarding the multi-variable bulk reconstruction procedure, which have not appeared in the author's previous publications. Part III concerns the application of the aforementioned results to study the finiteness of the F-theory flux landscape. Additionally, motivated by recent advances in the field of o-minimal geometry and the theory of unlikely intersections, we propose three conjectures which aim to address finer features of the flux landscape. Part IV investigates two corners of the landscape of 2d integrable non-linear sigma-models, namely the $\lambda$-deformed gauged WZW model and the critical bi-Yang-Baxter model. Notably, it is shown that asymptotic Hodge theory can be used to find broad classes of solutions these models.

==> appendices.tex <==
\chapter{Operator relations for Calabi-Yau fourfolds}\label{fourfold_rel}
In the construction of the sl(2)-approximation two operators $\eta$ and $\zeta$ appear, which can be expressed componentwise in terms of $\delta$ with respect to the decomposition \eqref{delta_decomp}. In this appendix we summarize these relations for Calabi-Yau fourfolds. For the purposes of this work we only need $\zeta$, but the expressions for $\eta$ are included for completeness.

Recall that the central identity relating the three operators was given by \eqref{delta-zeta-eta-review}. In the mathematics literature \cite{Kato} this was solved for the components of $\zeta$ for threefolds.\footnote{Furthermore, general expressions for the components $\zeta_{-p,-q}$ and $\eta_{-p,-q}$ in terms of $\delta_{-p,-q}$ were derived, modulo commutators of $\delta_{-r,-s}$ ($r\leq p$ and $s\leq q$) left undetermined.} These results were extended in \cite{Grimm:2021ikg}, where the components of $\eta$ were given in the threefold case. Following the strategy of these works \cite{Kato, Grimm:2021ikg}, we proceed and derive the componentwise expressions for $\eta$ and $\zeta$ for fourfolds. We refer to these articles for a more detailed explanation on how to work out these operator relations. We can express $\zeta$ componentwise in terms of $\delta$ as
\begin{footnotesize}
\begin{align}\label{fourfold_zeta}
 \zeta_{-1,-1}&= \zeta_{-2,-2}= 0\, , \quad \zeta_{-1,-2}= -\frac{i}{2} \delta_{-1,-2}\, , \quad \zeta_{-1,-3} = -\frac{3i}{4} \delta_{-1,-3}\, ,  \quad \zeta_{-1,-4} = -\frac{7i}{8} \delta_{-1,-4}\, ,\nn  \\
\zeta_{-2,-3} &=-\frac{3i}{8} \delta_{-2,-3}+ \frac{1}{8} [\delta_{-1,-2}, \delta_{-1,-1} ]\, , \qquad \zeta_{-2,-4} = -\frac{5i}{8} \delta_{-2,-4} + \frac{1}{4} [ \delta_{-1,-3}, \delta_{-1,-1} ]\, , \nn
\\
 \zeta_{-3,-3} &= \frac{1}{8}[\delta_{-2,-2}, \delta_{-1,-1}]\, ,  \\
\zeta_{-3,-4}  &= -\frac{5i}{16} \delta_{-3,-4} +\frac{3}{16} [\delta_{-2,-3} , \delta_{-1,-1} ] +\frac{3}{16} [\delta_{-1,-3}, \delta_{-2,-1} ] +\frac{i}{48} [\delta_{-1,-1}, [\delta_{-1,-1}, \delta_{-1,-2}]]\, ,  \nn \\
\zeta_{-4,-4} &= \frac{3}{16} [ \delta_{-3,-3}, \delta_{-1,-1} ] +\frac{3}{32} [\delta_{-3,-2} , \delta_{-1,-2}]+\frac{3}{32} [\delta_{-2,-3} , \delta_{-2,-1}]+\frac{i}{32} [\delta_{-1,-1}, [\delta_{-2,-1}, \delta_{-1,-2} ]] \, , \nn
\end{align}
\end{footnotesize}
while $\eta$ is expressed componentwise as
\begin{footnotesize}
\begin{align}\label{fourfold_eta}
\eta_{-1,-1} &= - \delta_{-1,-1}\, , \qquad \eta_{-1,-2} = - \delta_{-1,-2}\, , \qquad \eta_{-1,-3} = - \frac{3}{4}\delta_{-1,-3}\, , \qquad \eta_{-1,-4} = - \frac{1}{2}\delta_{-1,-4}\, , \nn \\
 \eta_{-2,-2} &= - \frac{3}{2} \delta_{-2,-2}\, , \hspace{125.5pt} \eta_{-2,-3} = -\frac{3}{2} \delta_{-2,-3}+\frac{i}{2} [\delta_{-1,-1}, \delta_{-1,-2}]\, , \nn  \\
 \eta_{-2,-4} &= -\frac{5}{4} \delta_{-2,-4}+\frac{5i}{8}[\delta_{-1,-1}, \delta_{-1,-3}]\, , \hspace{30.5pt} \eta_{-3,-3} =  -\frac{15}{8}\delta_{-3,-3}+\frac{5i}{4}[ \delta_{-2,-1}, \delta_{-1,-2}] \, , \nn \\
 \eta_{-3,-4} &= -\frac{15}{8} \delta_{-3,-4}+\frac{3i}{8}[ \delta_{-1,-1},  \delta_{-2,-3}]  \\
 &\quad+\frac{3i}{2}[ \delta_{-2,-1},  \delta_{-1,-3}]+\frac{3i}{4}[ \delta_{-2,-2},  \delta_{-1,-2}] +\frac{1}{8} [  \delta_{-1,-1}, [ \delta_{-1,-1},  \delta_{-1,-2}]]\, , \nn  \\
   \eta_{-4,-4} &= -\frac{35}{16} \delta_{-4,-4} +\frac{63i}{32} [\delta_{-3,-1}, \delta_{-1,-3}]+\frac{21i}{16} [\delta_{-3,-2}, \delta_{-1,-2}]+\frac{21i}{16} [\delta_{-2,-1}, \delta_{-2,-3}] \nn \\
   & \quad +\frac{7}{48}[\delta_{-1,-1},  [\delta_{-1,-1}, \delta_{-2,-2}]]+\frac{7}{24}[\delta_{-2,-1},  [\delta_{-1,-1}, \delta_{-1,-2}]]+\frac{7}{24}[\delta_{-1,-2},  [\delta_{-1,-1}, \delta_{-2,-1}]]\, . \nn
\end{align}
\end{footnotesize}

==> bulkreconstruction.tex <==
\chapter{Bulk Reconstruction in Moduli Space Holography}
%\section{Introduction}
%
%
%In recent years the study of general constraints on effective theories that can be coupled to quantized gravity has received 
%much attention, culminating in a vast network of `swampland conjectures' \cite{Palti:2019pca,vanBeest:2021lhn}. These conjectures
%have been mostly tested in string theory and highlight the observation that the known effective theories 
%arising from string theory are not generic. This should be contrasted with the fact that there is an immense number of 
%possibilities for connecting string theory with a four-dimensional theory, for example, by choosing different 
%compactification geometries. One approach to uncover the special properties of effective theories arising 
%from string compactifications is to consider the behaviour of their effective theories when taking limits in scalar field spaces. 
%This lead to a prominent set of swampland conjectures and emergence proposals \cite{Ooguri2007,Klaewer:2016kiy,GPV,Heidenreich:2018kpg,Lee:2019wij,Lanza:2020qmt,Calderon-Infante:2020dhm} 
%that describe the behaviour and validity of the effective theories when 
%moving to an asymptotic boundary after traversing an infinite geodesic distance. Furthermore, it is long known \cite{Ashok:2003gk,Acharya:2006zw} that 
%also finiteness statements about the number of flux vacua are dependent on the asymptotic behaviour of the effective theory 
%when approaching the boundary of field space. Taken together this provides motivation to develop new strategies to determine 
%and characterize the structure of field spaces and effective theories with a focus on their asymptotic properties. 
%
%Recently, it was proposed in  \cite{Grimm:2020cda} to develop a holographic description of the near-boundary effective theories. 
%More concretely, it was suggested that the properties of certain supersymmetric near-boundary effective theories 
%are determined holographically from a constrained set of boundary data and the solutions to an auxiliary bulk action principle \cite{Cecotti:2020rjq,Cecotti:2020uek,Grimm:2020cda}. This action is a non-linear sigma-model with a space-time that is 
%the field space, or rather moduli space, of the effective theory while the target space is a certain coset space built out of the 
%dualities and symmetries of the theory.  
%The most direct applications of these ideas lie in constraining the form of the vector sector in general 
%four-dimensional $\cN=2$ supergravity theories \cite{GPV,Cecotti:2020rjq,Cecotti:2020uek,Grimm:2020cda}. 
%More indirectly the holographic approach can also be applied for certain scalar potentials in $\cN=1$ supergravity actions that naturally 
%appear in flux compactifications \cite{Grimm:2019ixq,Grimm:2020cda}. There are two perspectives that one can take on this `moduli space 
%holography'. First, one can use it as an alternative way to study moduli spaces appearing in geometric compactifications of 
%string theory. Most notably, it applies rather directly to the moduli spaces of Calabi--Yau manifolds in any dimension and
%has been used to investigate various swampland conjectures, see e.g.  \cite{GPV,Grimm:2018cpv,Corvilain:2018lgw,Font:2019cxq, Grimm:2019wtx,Grimm:2019ixq,Lanza:2020qmt,Gendler:2020dfp,BastianGrimmHeisteeg,Grimm:2020ouv}. Second, it 
%can be viewed abstractly with no reference to any geometric realization and studied as a sigma-model whose solutions 
%with special boundary conditions admit some remarkable features. We will mostly take the latter perspective in this work, extend 
%the ideas of \cite{Grimm:2020cda}, and show that they are applicable in concrete examples.
%
%To give a concrete description of the model we constrain ourselves to an auxiliary matter bulk theory  
%with a space-time being a real two-dimensional manifold. The matter field is valued in a non-compact group $G_\bbR$, which preserves 
%a bilinear form on a finite-dimensional Hilbert space. Focusing on the non-linear sigma-model action for the matter fields, we find that it enjoys both global and local symmetries turning 
%the resulting target space into a coset construction reminiscent of a WZW model. 
%Being group-valued, the matter field acts as an operator on a finite-dimensional Hilbert space. One of the crucial aspects of the construction is that the Hilbert space enjoys a decomposition into a finite number of complex vector spaces, which can be thought of as assigning a background charge $Q$ to the various spaces. 
%In the geometric settings this corresponds to the Hodge decomposition of the cohomology groups of a K\"ahler manifold. 
%Much of the intricacy of our model comes from the interplay between the near-boundary behaviour of the bulk matter fields and the boundary charge decomposition of said Hilbert space. 
%Within this setting our aim is to find near-boundary solutions for the matter fields in a two-dimensional background metric that is flat up to a general overall Weyl factor. Furthermore, we require that the solutions admit a global continuous 
%symmetry, obey a special $Q$-constraint, and match a set of $\mathrm{Sl}(2,\mathbb{R})$ boundary conditions. The appearance of an $\SLt$-symmetry is consistent with the
%asymptotic behaviour of a natural metric on two-dimensional moduli spaces known as the Hodge metric.\footnote{Although we will not discuss the coupling to gravity of the model, we note that two different proposal for including gravity have appeared in \cite{Cecotti:2020uek} and \cite{Grimm:2020cda}, in which the Hodge metric plays an important role.} The latter can be constructed from the conserved currents associated to the global symmetry of the action, when evaluated on a solution to the equations of motion, and asymptotes to the Poincar\'e metric, which is invariant under an $\SLt$ isometry group. We will find that these 
%solutions admit remarkable properties and provide, in special geometric situations, asymptotic models for the periods of Calabi--Yau  
%manifolds. 
%
%
%
%
%A crucial restriction on the considered solutions is provided by the matching with a set of $\mathrm{Sl}(2,\mathbb{R})$ boundary data.  
%This boundary information consists of five special operators $Q_\infty, N^+, N^0, N^-$ and $\delta$, which act on, and define, the boundary Hilbert space. The charge operator $Q_\infty$ decomposes this  Hilbert space into various charge eigenspaces and 
%induces a well-defined inner product. 
%The operators $N^+, N^0$ and $N^-$ form a $\mathfrak{sl}(2,\mathbb{R})$-triple, which can be thought of as a completion 
%of the asymptotic global symmetry enjoyed by the considered set of solutions. By complexifying the algebra the $\slt$-triple can be used to further refine the split of the Hilbert space through a highest-weight decomposition that is compatible with the charge-decomposition. Finally, the phase operator  $\delta$ is crucial in order to uniquely fix the bulk solution. It controls the subleading corrections in the $1/y$ expansion of the 
%solutions with the boundary located at $y=\infty$. Note that the boundary data $Q_\infty,N^+, N^0, N^-$ together with the 
%sigma-model groups $G_\bbR$ can be classified 
%using $\SLt$-representation theory \cite{robles_2016,Kerr2017}. Within this vast set of possible boundary configurations we introduce a 
%special subclass that we call being of Calabi--Yau type. It will be these special types of boundary data that we later connect with period integrals 
%for a set of Calabi--Yau threefold examples. 
%
%With a detailed understanding of the bulk theory and boundary data, we set out to solve the equations of motion by reproducing large 
%parts of the proof of the $\SLt$-orbit theorem by Schmid \cite{Schmid} and Cattani, Kaplan, and Schmid (CKS) \cite{CKS}, albeit in a slightly different formulation. 
%We first note that the equations of motion of the bulk theory reduce to Nahm's equations when evaluated for the solutions satisfying 
%the specified asymptotic constraints. The strategy is to then decompose the bulk fields according to the charge associated to $Q_\infty$, and the weight and highest-weight associated to the $\mathfrak{sl}(2,\mathbb{C})$ acting on the Hilbert space at the boundary. This leads to a system of coupled recursion relations for the various components of the bulk field, which we term the CKS recursion relations \cite{CKS}. We will review 
%the $\SLt$-representation theory that ensures the recursive properties of these relations and recast them in a useful basis for explicit computations.  
%We then find that the recursion is so restrictive that the leading behaviour determined by the $\slt$-boundary condition, together with a single matching condition involving the phase operator, fixes all terms subleading in the near-boundary expansion uniquely. The construction of the near-boundary solutions starting 
%from the boundary data is reminiscent of the bulk reconstruction methods employed in the AdS/CFT duality \cite{Harlow:2018fse,Hamilton:2006az,Nakayama:2015mva}. We are considering massless fields, which simplifies the analysis, but note that the highly non-trivial structure arises due to the non-canonically normalized kinetic terms 
%in the action. This issue arises similarly in the holographic study of WZW models, see e.g.~\cite{Beccaria:2020qtk}. Let us stress that our approach differs both conceptually and technically from applying the AdS/CFT correspondence directly to the effective theories. This latter strategy has been successfully applied to testing swampland conditions in \cite{Nakayama:2015hga,Harlow:2015lma,Benjamin:2016fhe,Montero:2016tif,Montero:2017mdq,Harlow:2018tng,Harlow:2018jwu,Bae:2018qym,Conlon:2018vov,Montero:2018fns,Lin:2019kpn,Conlon:2020wmc,Ooguri:2020sua,Perlmutter:2020buo}.
%
%To elucidate these general consideration we will present a set of three simple examples with Calabi--Yau type boundary conditions. 
%We explicitly solve the CKS recursion relations and determine the bulk matter fields, containing all polynomially sub-leading corrections in powers of $1/y$ near the boundary $y=\infty$. We then explain how the bulk field solutions determine the asymptotic form of period integrals of general Calabi--Yau threefolds with a one-dimensional complex structure moduli space. In fact, we find that the three considered examples exactly capture the 
%three possible degenerations of such Calabi--Yau threefolds with unipotent monodromy, namely the conifold point, 
%the Tyurin degeneration, and the large complex structure point. This exemplifies the fact that a rather simple set 
%of algebraic boundary data fixes an infinite series of subleading corrections in the period vectors. 
%
%
%
%The paper is structured as follows. In section \ref{bulk-theory} we introduce the bulk theory defined on a real two-dimensional space-time. In particular, we write down an action for the bulk matter fields, discuss its symmetries and derive the equations of motion. We also describe some aspects of the geometry of the moduli space to motivate the particular class of solutions we will be considering. In section \ref{sec:boundary} we introduce the boundary data in detail and highlight the key properties that are required for the bulk reconstruction. Furthermore, the induced decomposition of the Hilbert space and its operators is discussed, together with a classification of the data. In table \ref{table:data} one may find the complete set of data that is used in this work. The main body of our work is comprised of sections \ref{Bulk-reconstruction} and \ref{reconstructing_examples}. In section \ref{Bulk-reconstruction} we give a detailed account of how the equations of motions are rewritten in terms of the CKS recursions and how the boundary data enters as an initial conditions in these recursions. Then in section \ref{reconstructing_examples} we solve the CKS recursion explicitly for the three examples. Finally, in section \ref{period_section} we describe the relation between the bulk fields and the period vector, by translating our description back to the Hodge-theoretical setting. There are two appendices. In appendix \ref{app:input} we have collected some computations on the $Q$-constraint and what it imposes on the input data of the CKS recursion. In appendix \ref{app:LCS_basis} one may find some explicit expressions that are used for the bulk reconstruction for $\mathrm{IV}_1$ boundaries.
%
%
%\section{The bulk theory}\label{bulk-theory}
%
%In this section we introduce the bulk matter theory and describe the set of solutions to the classical field 
%equations that will be studied in the remainder of this work. The bulk action is a two-dimensional non-linear sigma-model 
%of a group-valued matter field acting on a finite-dimensional Hilbert space and will be introduced in section \ref{bulk_matter_action}. 
%We discuss the symmetries of this theory and note that gauge equivalent matter field configurations live in a coset space $G_{\bbR} / M$. 
%In section \ref{local-solutions} we will then specify the considered asymptotic solutions that admit a global symmetry parametrized 
%by a nilpotent matrix $N^-$. These solutions turn out to be uniquely fixed by a set of boundary data consisting of an 
%sl$(2)$-algebra and two special operators, which are introduced later in section \ref{sec:boundary}. 
%
%Note that the constructions presented here are motivated by the behaviour of period maps from a moduli space 
%into the arithmetic quotients $\Gamma \backslash G_{\bbR} / M$. The considered action can be viewed as the two-dimensional 
%generalization of the action introduced in \cite{donaldson1984} that encodes Nahm's equations. It can also be derived as an 
%action encoding the $tt^*$ equations \cite{Cecotti:2020rjq}.   
%
%\subsection{The bulk matter action} \label{bulk_matter_action}
%
%In this section we introduce the bulk theory for a group-valued matter field $h$. It is given by a non-linear sigma-model 
%on a two-dimensional space $\cM$, the moduli space, and a target space being a real group $G_{\bbR}$. This real group 
%is defined by its action on some finite dimensional complex vector space $\cH$ and required to 
%preserve a bilinear product $\langle v , w \rangle$ on $\cH$, i.e.~we 
%require 
%\beq
%g\in G_{\bbR}:\quad \langle g v ,g w \rangle = \langle v , w \rangle\ . 
%\eeq
%Here we note that $G_{\bbR}$ need not comprise the full symmetry group of the bilinear product. To define the sigma-model, we also introduce a special  inner product $\langle v|w \rangle$, which renders 
%$\cH$ into a Hilbert space. This inner product is induced by an operator $Q \in i\mathfrak{g}_{\bbR}$ that defines 
%a split of $\cH$ into $D+1$ vector spaces
%\beq
%\cH_q\ , \quad q=-\frac{D}{2}, -\frac{D}{2}+1,..., \frac{D}{2}\ , 
%\eeq
%where $D$ will be called the \textit{weight} associated to the Hilbert space $\cH$. 
%We can think of $q$ as being the charge 
%of a state in $\cH_q$, i.e.~we have 
%\beq \label{ref-Q}
%|w\rangle \in \cH_q:   \quad  Q |w\rangle =q |w\rangle \ ,
%\eeq
%where we have used bra-ket notation to denote states in $\cH$. 
%Note that by definition $\bar Q = - Q$, which implies that all eigenstates with non-vanishing real charge are complex.
%Given such a charge operator $Q$ the inner product  $ \langle v|w \rangle$  is defined as 
%\beq \label{def-innerproduct}
%\langle v|w \rangle :=  \langle \bar v, e^{\pi i Q} w \rangle\ .
%\eeq
%This inner product allows us to associate to each operator $\cO$ acting on $|w \rangle$ an 
%adjoint operator $\cO^\dagger$. 
%
%We are now in the position to introduce the sigma-model action for the fields $h$. In order to do this 
%we denote by $\sigma^\alpha$,  $\alpha =1,2$ real local coordinates on $\cM$ and define $g_{\alpha \beta}$ to be 
%a background metric on $\cM$. The action that we consider for the matter field takes the form  
%\beq \label{Smat_1}
%S_{\rm mat}(h) = \frac{1}{4}\int_{\cM} d^2 \sigma \sqrt{g} g^{\alpha \beta} \mathrm{Tr}\left(h^{-1} \partial_\alpha h+\left(h^{-1} \partial_\alpha h\right)^\dagger \right)\left(h^{-1} \partial_\beta h+\left(h^{-1} \partial_\beta h\right)^\dagger \right)\ ,
%\eeq
%where the trace is evaluated by using the inner product $ \langle v|w \rangle$ defined in \eqref{def-innerproduct}. It will 
%later be useful to employ form notation on $\cM$, writing e.g.~$\dd h = \partial_\alpha h \, \dd \sigma^\alpha$. The action \eqref{Smat_1}
%can then be written more compactly as 
%\begin{equation}\label{Smat_2}
%S_{\rm mat}(h) = \frac{1}{4}\int \mathrm{Tr}\left| h^{-1} \text{d} h+\left(h^{-1} \text{d} h\right)^\dagger \right|^2\ ,
%\end{equation} 
%where $|A|^2 = A \wedge * A$ with $*$ being the Hodge star on $\cM$ in the background metric $g_{\alpha \beta}$.  Let us stress that $h$ is a group-valued field and thus, in general, combines the degrees of freedom of multiple massless scalar fields. Due to the non-linearity of the action \eqref{Smat_2} in $h$ any simple parametrization of $h$ in terms of scalar fields will result in non-canonically normalized kinetic terms, which highlights the complexity of the model.
%
%Let us point out that this action has two sets of symmetries, which we will discuss in turn. Firstly, we see that \eqref{Smat_2}
%has a global invariance under left-multiplication 
%$h(\sigma) \rightarrow g_L h(\sigma) $ with $g_L \in G_{\bbR}$.
%This global symmetry yields  a conserved current of the form
%\begin{equation}
%\label{eq:current}
%J_L = \frac{1}{2} *\big[(\text{d}h)h^{-1}+h\left(h^{-1}\text{d}h\right)^\dagger h^{-1}\big]\ .
%\end{equation}
%Secondly, one checks that \eqref{Smat_2} has a local invariance under right-multiplication 
%$h(\sigma) \rightarrow h(\sigma) g_R(\sigma)$, with $g_R^\dagger(\sigma) = g^{-1}_{R}(\sigma)$. 
%The presence of this gauge symmetry shows that the matter action \eqref{Smat_2} actually 
%describes fields in a coset $G/M$, where $M$ consists of the group elements $g_R$ that satisfy the unitarity condition
%$g_R^\dagger = g^{-1}_{R}$ with respect to the inner product \eqref{def-innerproduct}. Put differently, $M$ can be realized as the stabilizer of the group element $e^{\pi i Q}$.\footnote{For this one uses the fact that $g^\dagger = e^{-\pi iQ}g^{-1} e^{\pi i Q}$ for a group element $g\in G$, cf. \eqref{def-innerproduct}} It is a general result that this always yields a maximal compact subgroup of $G$. In fact, the converse is also true: to each maximal compact subgroup of $G$ one can associate an inner product which is stabilized by it \cite{Borel1973}.

%\subsection{Near-boundary solutions at the center of the Poincar\'e disc} \label{local-solutions}
%
%We now turn to the study of the solutions to the classical equations of motion 
%of the matter action \eqref{Smat_2}. Concretely, we will consider a background 
%metric with the line element 
%\beq \label{conformally-flat}
%g_{\alpha \beta} d\sigma^\alpha d\sigma^\beta = f^2(\sigma) \big[(d\sigma^1)^2 + (d\sigma^2)^2 \big]\ , 
%\eeq
%where $f(\sigma)$ is a (non-vanishing) function of $\sigma$. It is easy to check that the Weyl factor 
%$f^2$ drops from the action and the equations of motion. As long as we do not couple this theory 
%to two-dimensional gravity, we are thus free to work with any choice of $f(\sigma)$. 
%
%\begin{figure}[h!]
%	\begin{center}
%		\includegraphics[width=0.8\textwidth]{disc_fig.pdf}
%		\vspace*{-1cm}
%	\end{center}
%	\begin{picture}(0,0)
%	\put(70,82){\rotatebox{-31}{\small $z \rightarrow 0$}}
%	\put(307,88){\small $y \rightarrow \infty$}
%	\put(10,110){(a)}
%	\put(200,110){(b)}
%	\end{picture}
%	
%	\caption{Local patch in the space $\cM$ represented as Poincar\'e disc, Figure (a), and upper half-plane, Figure (b). 
%		The asymptotic solutions  are expanded near the boundary at $z=0$ in the disc, which is mapped to 
%		$t = i \infty$ on the upper half plane. \label{fig:disc}}
%	
%\end{figure}
%
%
%
%In the following we will consider a local patch in $\cM$ that can be represented by 
%the punctured Poincar\'e unit disc or its universal cover, the upper half plane. We will 
%be interested in determining solutions near the puncture of the disc, which is mapped 
%to imaginary infinity in the upper half plane, as depicted in Figure \ref{fig:disc}. 
%Working on the disc we pick complex coordinates $z,\bar z$, such that $0<|z|\leq 1$, with the puncture 
%located at $z=0$. The upper half plane covering the disc can be parametrized 
%by introducing coordinates $t=\frac{1}{2\pi i} \log z = x + i y$. 
%The metric on the upper half plane can be taken 
%to be the standard Poincar\'e metric given by 
%\beq  \label{Poincare-metric}
%g^{\text{\tiny Poincar\'e}}_{\alpha \beta}\,  d\sigma^\alpha d\sigma^\beta = \frac{1}{y^2} \big[(d x)^2 + (dy)^2 \big]\ , \qquad \sigma^1=x, \ \sigma^2 = y\ . 
%\eeq
%We note that the precise form of this metric will be relevant when attempting to couple the matter 
%theory \eqref{Smat_2} to a two-dimensional gravity theory that is not Weyl invariant. 
%
%Two proposals of coupling of the matter action \eqref{Smat_2} to a gravity theory have been studied in \cite{Cecotti:2020uek} and \cite{Grimm:2020cda}. In both constructions a 
%special metric on the moduli space, the so-called Hodge metric, played a central role. To see how this metric 
%arises from our general perspective, let us note that one can construct a natural metric $g_{\alpha\beta}(J_L)$ on $\cM$ using the conserved currents \eqref{eq:current} as 
%\begin{equation}\label{eq:hodgemetric}
%g_{\alpha\beta}(J_L) d\sigma^\alpha d\sigma^\beta= \mathrm{Tr}\left[ (J_L)_\alpha (J_L)_\beta \right]d\sigma^\alpha d\sigma^\beta \ ,
%\eeq
%where $(J_L)_\alpha$ denotes the $\alpha$-component of the 1-form $J_L$.
%We will show in section \ref{ssec:reconstructmetric} that one can evaluate this metric on a solution of the bulk matter theory and find the general asymptotic form 
%\beq \label{eq:metricexpand}
%g_{\alpha\beta}(J_L^{\rm sol}) d\sigma^\alpha d\sigma^\beta=  \frac{1}{y^2}\left( c^{(0)}+ \frac{c^{(1)}}{y}+\frac{c^{(2)}}{y^2}+\cdots\right) \big[(d x)^2 + (dy)^2 \big]\ .
%\end{equation}
%We find that for all our solutions $ c^{(0)} \neq 0$, such that the metric has the leading asymptotic 
%behaviour of the Poincar\'e metric \eqref{Poincare-metric}. In fact, we will see that concrete expressions for the coefficients $c^{(i)}$ can be derived in terms of the boundary data in \eqref{eq:ci}. It was argued in \cite{Cecotti:2020uek,Grimm:2020cda} that in geometric settings the metric $g_{\alpha\beta}(J_L^{\rm sol}) $ coincides with the Hodge metric. 
%
%Let us now return to analyzing the near-boundary solutions for the bulk theory we have introduced. Evaluating the equations of motion of the action \eqref{Smat_2} in a metric of the form \eqref{conformally-flat}
%yields the equation
%\beq \label{eom_in_flat_gauge}
%\sum_\alpha \partial_{\sigma^\alpha}  \big(  h^{-1}  \partial_{\sigma^\alpha}   h + ( h^{-1}  \partial_{\sigma^\alpha}   h)^\dagger \big) - \big[(  h^{-1} \partial_{\sigma^\alpha}   h)^\dagger,   h^{-1} \partial_{\sigma^\alpha}   h \big] = 0\ .
%\eeq
%Our aim is to determine solutions to this equation near the boundary $y=\infty$. 
%The class of solutions that we determine is constrained by a number of conditions. Firstly, we 
%note that $h(z,\bar z)$ can transform under a monodromy transformation when encircling the center 
%of the disc. More precisely, such a transformation would rotate
%\beq
%h(z,\bar z) \ \rightarrow \ T h(z,\bar z)\ , 
%\eeq
%when sending $z \rightarrow e^{2\pi i }z$. 
%Here $T$ is an element of the monodromy group $\Gamma \subset G_{\mathbb{R}}$ of $\cM$.  
%The fields $h(z,\bar z)$ are thus single-valued if we work on the quotient $G_{\bbR}/\Gamma$.
%In the following we will assume that $T$ is unipotent, i.e.~that it 
%can be written as 
%\beq \label{nil_mod}
%T = e^{N^-}\ , 
%\eeq
%where $N^-$ is a nilpotent matrix $(N^-)^k = 0$, $k>D$. When formulated in terms of the coordinates 
%$t = x + i y$ on the covering space of $\cM$, the matter fields $h$ thus behave as 
%\beq \label{discrete_sym}
%h(x+ 1,y) = e^{N^-} h(x, y)\ .
%\eeq
%Clearly, we can obtain this transformation behaviour by setting $h(x,y) = e^{xN^-} \tilde h(x,y)$ with $\tilde h(x,y)$ being a periodic function invariant under the shift $x \rightarrow x+1$. In the following we will require that sufficiently close to the puncture the 
%discrete symmetry \eqref{discrete_sym} becomes continuous, i.e.~that  $x \rightarrow x + c$ for any constant $c$ 
%is a symmetry of the action \eqref{Smat_2}. Together with \eqref{discrete_sym} this implies that $h$ is of the form 
%\beq \label{h-split-form}
%h(x,y) = e^{x N^-} \tilde h(y)\ .
%\eeq
%Solving the equations of motions \eqref{eom_in_flat_gauge} we will thus have to solely determine the $G_\bbR$-valued function $\tilde h(y)$.

%Finding solutions of \eqref{eom_in_flat_gauge} that take the form \eqref{h-split-form} is still a notoriously difficult task. One additional constraint 
%that we will impose is a compatibility condition of such solutions with $Q$. Concretely, we will demand that 
%\beq \label{Q-constraint}
%-2\big[Q,  h^{-1} \partial_{y}   h\big]= i \Big( (  h^{-1} \partial_{x}   h)^\dagger +    h^{-1} \partial_{x}   h \Big) \ , \qquad     \big[Q,  h^{-1} \partial_{x}   h \big] =i  h^{-1} \partial_{y}   h \ . 
%\eeq 
%These conditions imply that $ (  h^{-1} \partial_{y}   h)^\dagger =   h^{-1} \partial_{y}  h $.
%
%We are now in the position to summarize the equations that we will solve recursively in the remainder of this paper. First, we introduce the following shorthand notation
%\beq  \label{def-cN}
%\cN^0(y) := - 2   h^{-1}  \partial_y   h\ ,  \qquad \cN^-(y)  :=    h^{-1}  \partial_x   h \ ,\qquad
%\cN^+(y)  := (\cN^-(y))^\dagger\ .
%\eeq
%It is then straightforward to check that \eqref{eom_in_flat_gauge} together with \eqref{Q-constraint} imply the 
%differential equations 
%\beq \label{Nahm_eq}
%\partial_{y} \cN^{\pm} = \pm \tfrac{1}{2} [\cN^{\pm},\cN^0] \ , \qquad  
%\partial_{y} \cN^0 =- [\cN^{+} ,\cN^{-}]\ ,
%\eeq
%and the algebraic conditions 
%\beq \label{Q-constr_2}
%\big[Q,\cN^{0}\big]= i  (\cN^+ + \cN^-) \ , \qquad     \big[Q,\cN^{\pm}\big] =-\tfrac{i}{2} \cN^0 \ . 
%\eeq
%Note that the differential equations \eqref{Nahm_eq} are also known as Nahm's equations. The two equations on the left are automatically solved for $\cN^0,\cN^\pm$ of the form \eqref{def-cN}, while the equation on the right 
%corresponds to the equations of motion \eqref{eom_in_flat_gauge}.
%
%
%
%\section{The boundary data}
%\label{sec:boundary}
%
%In this work we will consider solutions to the equations \eqref{Nahm_eq}, \eqref{Q-constr_2} and determine bulk fields that are of the 
%general form \eqref{h-split-form}. We note, however, that these conditions do not fix the bulk solutions entirely. In section \ref{sec:boundary_theory} a set of boundary data is introduced, which fixes the solution uniquely upon imposing a single matching condition \eqref{zetadelta-eq} as is explained in section \ref{Bulk-reconstruction}. We then provide a classification of this boundary data  in section \ref{boundary_class} for boundaries of Calabi--Yau type with $D=3$. This classification applies to moduli spaces of any dimension, and when restricting to two-dimensional moduli spaces there will remain only three non-trivial possibilities, which we call type $\mathrm{I}_1$, $\mathrm{II}_0$ and $\mathrm{IV}_1$. We construct the most general set of boundary data for these three types of boundaries in section \ref{ssec:data}, which will be the starting point for the examples we study later. 
%
%\subsection{The sl(2) boundary data}
%\label{sec:boundary_theory}
%We start by discussing the general aspects of the boundary data. The following structures can be extracted from the Hodge theory constructions of \cite{Schmid,CKS}. We follow here the presentation of \cite{Grimm:2020cda}, which states 
%the relevant information without reference to Hodge structures. From the mathematical perspective the following presentation uses ideas 
%put forward in \cite{robles_2016}. To begin with we require that the vector space $\cH$ also admits a splitting into vector spaces $\cH^\infty_q$ that is attached to the boundary at $y=\infty$. We encode this splitting by a boundary charge operator $Q_\infty\in i\mathfrak{g}_{\mathbb{R}}$
%\begin{equation}\label{eq:Qdecomp}
%|w\rangle \in \cH^\infty_q:\quad Q_\infty |w\rangle = q |w\rangle\ .
%\end{equation}
%In order to find well-behaved solutions $h$ that match this boundary splitting, we require that $Q_\infty$ is 
%at most a rotated version of the charge operator $Q$ introduced in \eqref{ref-Q}. Concretely, we require that there exists a 
%$\zeta \in \mathfrak{g}_{\mathbb{R}}$ such that $Q = e^{-\zeta} Q_\infty e^{\zeta}$.
%From $Q_\infty$ one may again construct an inner product via
%\begin{equation}
%\langle v | w \rangle_\infty := \langle \bar{v}, e^{i\pi Q_\infty} w\rangle\ .
%\end{equation}
%which is simply a rotated variant of the inner product introduced in \eqref{def-innerproduct}. 
%
%The second structure that we require to exist on the boundary is an $\slt$-algebra of operators acting on $\cH$. Recall that we associated a nilpotent matrix $N^-$ to the puncture in \eqref{nil_mod}. Also note that there are many ways to pick two other generators $N^+$, $N^0$ such that 
%the triple $N^\pm, N^0\in\mathfrak{g}_{\mathbb{R}}$ commute as $\slt$ generators. The crucial point here is that we consider a choice that 
%is compatible with the splitting induced by $Q_\infty$
%We will formulate the properties of this algebra both in the real and complex setting. The real algebra $\mathfrak{sl}(2,\mathbb{R})$ is generated by $N^\pm, N^0\in\mathfrak{g}_{\mathbb{R}}$ and the complex algebra is generated by $L_{\pm 1}, L_0\in\mathfrak{g}_{\mathbb{C}}$, satisfying the commutation relations
%\begin{equation} \label{real-sl2alg}
%[N^0, N^\pm] = \pm 2N^\pm, \quad [N^+, N^-]=N^0,
%\end{equation}
%and
%\begin{equation}
%[L^0, L_{\pm 1}] =\pm  2L_{\pm 1}\, , \quad [L_{1}, L_{-1}]=L_0\, .
%\end{equation}
%The two sets of generators are related by
%\begin{equation}\label{eq:Ldef}
%L_{\pm 1} =\frac{1}{2}\left(N^+ + N^- \mp i N^0 \right),\quad L_0 = i\left(N^- - N^+\right).
%\end{equation}
%It turns out that there is another way to describe the relation between $N^0,N^\pm$ and $L_0,L_{\pm 1}$, namely by 
%a transformation with a group element $\rho \in G_\bbC$ defined as
%\begin{equation} \label{def-rho}
%\rho=\mathrm{exp}\Big[\frac{i\pi}{4}\big(N^+ + N^-\big)\Big]=\mathrm{exp}\Big[\frac{i\pi}{4}\left(L_{1} + L_{-1}\right)\Big]\ .
%\end{equation}
%It is not hard to check\footnote{Here one can use the identity for the adjoint actions $\text{Ad}_{\text{exp} \cO} =  \text{exp}(\text{ad}_\cO)  $.} that $\rho$ allows us to move between the real and complex algebra via
%\begin{equation}
%\label{eq:rho_switch}
%L_{\pm 1} = \rho N^\pm \rho^{-1}\, ,\quad L_{0} = \rho N^0 \rho^{-1}\, .
%\end{equation}
%The compatibility with $Q_\infty$ can be formulated as
%\begin{equation}
%[Q_\infty, N^0] = i\left(N^++N^-\right), \quad [Q_\infty, N^\pm] = -\frac{i}{2}N^0\, ,
%\end{equation}
%or
%\begin{equation}
%[Q_\infty, L_\alpha] =\alpha L_\alpha \,,\quad \alpha = \pm 1,  0 \, .
%\end{equation}
%A crucial observation is that $L_0$ commutes with $Q_\infty$, which allows us to find a common eigenbasis for the two operators. For this reason we will mostly work with the complex algebra. There is, of course, one more operator which commutes with both $L^0$ and $Q_\infty$, namely the Casimir operator $L^2$. It is given by
%\begin{equation} \label{def-Casimir}
%L^2=2L_{1}L_{-1} + 2L_{-1} L_{1} +(L_0)^2 \, .
%\end{equation}
%Let us note that there is another way of interpreting the operators $L^\alpha, Q_\infty$. In fact, we see that 
%$\hat Q \equiv  Q_\infty - \frac{1}{2} L_0$ commutes with all $L_{\alpha}$ and hence we have the algebra 
%\beq
%\mathfrak{sl}(2,\bbR) \oplus \mathfrak{u}(1): \ L^\alpha, \hat Q\ . 
%\eeq
%in this work we prefer to work with the charge operator $Q_\infty$ instead of $\hat{Q}$, but note that $\hat{Q}$ does appear naturally in the bulk reconstruction in e.g.~\eqref{charges_cL}.
%
%Much of our work revolves around solving operator equations, hence it will be extremely useful to split the space of operators using the eigenvalues of $L^2, L^0$ and $Q_\infty$. Concretely, given any operator $\cO $ we may decompose it as
%\beq \label{weight-charge-expansion-operator1}
%\cO = \sum_{0 \leq d \leq D} \sum_{-d\leq s\leq d} \sum_{-D\leq q \leq D} \cO^{(d,s)}_q \ , 
%\eeq
%with 
%\bea \label{weight-charge-expansion-operator2}
%(\ad L)^2 \cO^{(d,s)}_q &=& d(d+2)\, \cO^{(d,s)}_q  \ , \nn \\
%\big[L_0,\cO^{(d,s)}_q\big] &=&  s\, \cO^{(d,s)}_q\ ,  \\
%\big[Q_\infty ,\cO^{(d,s)}_q \big] &=& q\, \cO^{(d,s)}_q\ ,  \nn 
%\eea
%where we have used the shorthand notation $(\ad L)^2$ to denote replacing each left-multiplication in \eqref{def-Casimir} with an 
%adjoint action, i.e.~we have set
%\beq
%(\ad L)^2 \cO :=2\big[L_{1},\big[L_{-1},\cO \big]\big]+2\big[L_{-1},\big[L_{1},\cO \big]\big]+\big[L_0,\big[L_0,\cO \big]\big]\ .
%\eeq
%We call $d, s$ and $q$ the \textit{highest weight}, \textit{weight} and \textit{charge} of the operator, respectively. 
%In the following, it is sometimes not necessary to perform all three decompositions \eqref{weight-charge-expansion-operator2}.
%We will then employ the notation
%\beq \label{weightonly}
%\cO^{(l)}_q \equiv  \sum_{d \in \bbZ} \cO^{(d,l)}_q\ ,\qquad \cO^{(d,l)} \equiv  \sum_{q \in \bbZ} \cO^{(d,l)}_q \ , \qquad \cO^{[d]} \equiv  \sum_{q,l \in \bbZ} \cO^{(d,l)}_q \ ,
%\eeq
%when we do not perform the highest weight decomposition, the charge decomposition, or only perform the highest weight decomposition, respectively.
%
%Note that in the case we do not perform a charge decomposition, one could also have chosen to perform the highest weight and weight decomposition with respect to the real $\slt$-algebra \eqref{real-sl2alg}. 
%These two decompositions are related precisely by $\rho$ introduced in \eqref{def-rho}. In other words, if $\cO$ is an operator with weight $s$ under $N^0$, then $\hat{\cO}=\rho\cO\rho^{-1}$ is an operator with weight $s$ under $L^0$, and similarly for the highest weight. In the following we will add a hat to an operator if it is obtained via the transformation with $\rho$. This is particularly relevant if $\cO$ is a real operator. Such operators are naturally decomposed with respect to the real $\slt$-algebra \eqref{real-sl2alg} and cannot be an eigenoperator under $Q_\infty$, unless they are uncharged.  
%
%The last boundary operator that we need to introduce is a real operator $\delta \in \mathfrak{g}_{\mathbb{R}}$. It is an essential part of the boundary data and determines crucially the complexity of the associated bulk solutions. We will call this operator the \textit{phase operator} as in ref.~\cite{Grimm:2020cda}. In accordance with the notation introduced above, we use $\delta$ to define
%\begin{equation}
%\hat{\delta} = \rho\delta\rho^{-1} \ ,
%\end{equation} 
%which is thus an element of $ \mathfrak{g}_{\bbC}$.
%The phase operator $\delta$ or $\hat{\delta}$ is required to have a number of special properties such that it can be part of a consistent set of boundary data. 
%Firstly, it has to commute with $L_{-1}$, i.e.~we require
%\begin{equation}
%\label{eq:delta_Lmin}
%[L_{-1},\hat{\delta}]=0\ .
%\end{equation}
%Secondly, its components all have weight less than or equal to $-2$, and charge less than or equal to $-1$. In other words, we require that 
%it admits an expansion
%\begin{equation}\label{eq:deltaexpansion}
%\hat{\delta} = \sum_{s\leq -2} \sum_{q \leq -1} \hat{\delta}^{(s)}_q\ .
%\end{equation}
%We will show in section \ref{Bulk-reconstruction} that these properties of the phase operator $\delta$ suffice to fix the associated bulk solution uniquely 
%after imposing one matching condition. 
%
%\subsection{Classifying boundary data} \label{boundary_class}
%The data we have just introduced can now be used to classify the boundary data. Recall that a given boundary is characterized by an $\mathfrak{sl}(2,\mathbb{C})$-triple $(L_1,L_0,L_{-1})$, a charge operator $Q_\infty$ and a phase operator $\delta$. Since the boundary operators lie in the algebra of $G_{\bbR}$, it is important to stress the dependency of $G_{\bbR}$ on the choice of the bilinear $\langle \cdot, \cdot \rangle$. Moreover, since $G_{\bbR}$ need not comprise the full symmetry group of the bilinear, there are many choices that can be made, which greatly complicates the classification. Nevertheless, a full classification of allowed groups $G_{\bbR}$ and boundary data has been given by Robles in \cite{robles_2016}. As part of this classification one has to classify the charge operator and $\slt$-triple based on the eigenvalues of the weight operator $L_0$, the Casimir $L^2$ and the charge operator $Q_\infty$. This classification then captures what spectra are allowed for the operators $L^2,L^0$ and $Q_\infty$ in order to obtain a consistent boundary theory. In other words, it tells us which splittings of the vector space $\cH$ into eigenspaces of these operators have to be considered, which allows us to systematically go through all possible cases.
%
%Let us begin with the splitting of the vector space $\cH$
%induced by the charge operator $Q_\infty$ into $D+1$ eigenspaces as in \eqref{eq:Qdecomp}, and gather the dimensions of these eigenspaces $\cH^\infty_q$ together as
%\begin{equation} \label{H-dimq}
%\dim \cH^\infty_q = (h_{D/2},\, h_{D/2-1}, \, \ldots,\, h_{-D/2+1},\, h_{-D/2} )\, ,
%\end{equation}
%These dimensions satisfy $h_{q}=h_{-q}$, since under complex conjugation the eigenspaces are related by $\overline{\cH}_{q}=\cH_{-q}$. 
%The splitting of the vector space $\cH$ into eigenspaces $\cH^{\infty}_{q}$ is then refined by considering the $\mathfrak{sl}(2,\mathbb{C})$-triple $(L_1,L_0,L_{-1})$. The weight and Casimir operators $L_0,\, L^2 $ commute with the charge operator $Q_\infty$, so the vector space $\cH$ admits a common eigenbasis. We therefore decompose each eigenspace $\cH^\infty_q$ as
%\begin{equation} 
%\cH^\infty_q = \sum_{0\leq d \leq D} \sum_{-d \leq s \leq d} \left(\cH^\infty \right)_q^{(d,s)}\, , 
%\end{equation}
%where for an element $|d,s;q\rangle  \in \left(\cH^\infty \right)_q^{(d,s)}$ one has
%\begin{equation}\begin{aligned}
%L_0 |d,s;q\rangle  &= s |d,s;q\rangle\, , \\
%L^2 |d,s;q\rangle &= d(d+2) |d,s;q \rangle\, , \\
%Q_\infty |d,s;q\rangle  &= q |d,s;q \rangle \, . \\
%\end{aligned}\end{equation}
%One can now use this refined splitting to classify the boundary data. While we will present in section \ref{Bulk-reconstruction} the general formalism to solve the bulk theory for any boundary data, our explicit examples in section \ref{reconstructing_examples} will consist of data of a distinguished type, which we call being of Calabi--Yau type:\footnote{In this setting the $h_q$ are related to the Hodge numbers $h^{p,q}=\mathrm{dim}_\mathbb{C}\; H^{p,q}(Y_D,\mathbb{C})$ by $h^{p,q}=h_{(p-q)/2}$.}
%\beq \label{CYtype-cond}
%\text{Calabi--Yau type:} \quad h_{D/2}=h_{-D/2}=1\, , \qquad G_{\bbC}=
%\begin{cases}
%	\mathrm{Sp}(\dim\cH, \bbC)\, ,& D \,\mathrm{ odd }\, ,\\
%	\mathrm{SO}(\dim\cH, \bbC)\, , & D\, \mathrm{ even }\, .
%\end{cases}
%\eeq
%From a geometric perspective the first condition is related to the fact that there exists a unique holomorphic $(D,0)$-form on a Calabi--Yau manifold
%of complex dimension $D$. The second condition implies that $G_{\bbR}$ comprises the full symmetry group of the bilinear form $\langle\cdot,\cdot\rangle$, which is (skew-)symmetric for (odd) even $D$. In particular, we will consider the case $D=3$. For this reason it will be sufficient to review only part of the classification, restricting to the case where we have dimensions $(1,h_{1/2},h_{1/2},1)$ and group $G_{\bbR}=\mathrm{Sp}(2+2h_{1/2},\bbR)$ as in \cite{Kerr2017,Grimm:2018cpv}. 
%
%Based on the eigenvalue of $\cH^\infty_{3/2}$ under $L_0$ we separate into four principal types by
%\begin{equation}\label{eq:principaltypes}
%\left| \hat{d}, \hat{d} ; \tfrac{3}{2} \right\rangle \in  \cH^\infty_{3/2}\ , \qquad \begin{cases}
%\mathrm{I}&: \qquad \hat{d}=0\, ,\\
%\mathrm{II}&: \qquad \hat{d}=1\, ,\\
%\mathrm{III}&: \qquad \hat{d}=2\, , \\
%\mathrm{IV}&: \qquad \hat{d}=3\, .
%\end{cases}
%\end{equation}
%Alternatively this condition can be phrased as that the lowering operator $L_{-1}$ (or $N^-$) can act at most $\hat{d}$ times on an element in the $q=3/2$ eigenspace before vanishing, since it is part of a $(\hat{d}+1)$-dimensional irreducible representation. Note that $\hat{d}$ is at most equal to three, since applying $L_{-1}$ also lowers the charge of the state, and $q\geq -\frac{3}{2}$ when $D=3$. 
%
%In the same spirit we can characterize how the $q=1/2$ eigenspace decomposes under the operators $L^2$ and $L_0$. Note that the decomposition of the $q=-1/2$ and $q=-3/2$ eigenspaces then follows by complex conjugation. We can encode the splitting of $\cH^\infty_{1/2}$ by a single integer $n$ defined as
%\begin{equation}
%\label{eq:secondary_type}
%n = \sum_{0\leq d \leq 3} \dim \left(\cH^\infty \right)_{1/2}^{(d, 1)}.
%\end{equation}
%In other words, $n$ denotes the number of linearly independent states with weight $s=1$ and charge $q=1/2$. It turns out that the principal type and the integer $n$ together classify all types of boundary splittings of $\cH$, which we denote by\footnote{This classification naturally applies to limits in the complex structure moduli space of Calabi--Yau threefolds, and by using mirror symmetry it can be used to characterize limits in K\"ahler moduli spaces \cite{Grimm:2018cpv,Corvilain:2018lgw}. In turn, it was suggested in \cite{Grimm:2019bey} that the limit types on the K\"ahler cone can be combined into graphs to classify the Calabi--Yau threefolds themselves.} 
%\begin{equation}
%\mathrm{I}_n\, , \quad \mathrm{II}_n\, , \quad \mathrm{III}_n \, ,  \quad \mathrm{IV}_n\, .
%\end{equation} 
%Here the range for the index $n$ changes per principal type and depends on the value of $h_{1/2}$. For example, for type $\mathrm{IV}_n$ there is at least one vector with weight $s=1$ and charge $q=1/2$, namely $L_{-1}|3, 3;3/2\rangle$,  hence $n\geq 1$. On the other hand, $n$ cannot exceed the dimension of $\cH^\infty_{1/2}$, so $n\leq h_{1/2}$. One can consider the other principal types in a similar fashion to arrive at the following ranges
%\begin{align} \label{general-types_3}
%\mathrm{I}_n&:\quad 0\leq\; n \leq h_{1/2}\, , &
%\mathrm{II}_n&:\quad 0\leq \;n \leq h_{1/2}-1 \, ,& \\
%\mathrm{III}_n&:\quad 0\leq \;n \leq h_{1/2}-2 \, ,&
%\mathrm{IV}_n&:\quad 1\leq \;n\leq h_{1/2}\ . &
%\end{align}
%To close our discussion, let us point out that the phase operator $\delta$ is not captured by the classification of the boundary data that we have just reviewed. 
%While it is a crucial element of the set of boundary data, it is not involved in the splitting of the vector space $\cH$ into eigenspaces under the operators $Q_\infty, L^2, L_0$. Given this data, the phase operators $\delta$ then has to be an operator acting on this splitting that satisfies \eqref{eq:delta_Lmin} and \eqref{eq:deltaexpansion}. In the next subsection we discuss the simplest situation with $h_{1/2} = 1$ in which the phase operators can 
%be parameterized easily. 
%
%\subsection{Classifying phase operators in simple Calabi--Yau type settings}
%\label{ssec:data}
%
%Having briefly reviewed the classification of the boundary data associated to $Q_\infty, L^2, L_0$, we now want to have a closer look 
%at a certain set of special cases. More precisely, we will consider boundary data of Calabi--Yau type and weight $D=3$, which 
%also satisfies the condition $h_{1/2} = 1$. This latter assumption will be particularly useful when identifying the allowed phase operators 
%$\delta$ compatible with the algebra obtained from $Q_\infty$, $L_\alpha$. 
%It follows from \eqref{general-types_3} that there are only three possible non-trivial types, namely
%\begin{equation} \label{simple-types}
%\quad h_{3/2}=h_{1/2}=1:\quad \mathrm{I}_1\, ,\quad \mathrm{II}_0\, ,\quad \mathrm{IV}_1 \ . 
%\end{equation}
%In a geometric realization these boundary data can arise in the complex one-dimensional moduli space of a Calabi--Yau threefold. 
%The boundary types respectively cover the conifold point, the Tyurin degeneration, and the large complex structure point as we will 
%see in detail in section \ref{reconstructing_examples}. We exclude type $\mathrm{I}_0$ because it corresponds to the trivial representation where $L_{-1}=0$.
%
%In the following we explicitly determine the boundary data associated to the types \eqref{simple-types}. The reader can find the result in table \ref{table:data}. To begin with, recall that for the three boundary types under consideration the group $G_{\mathbb{R}}$ is given by the symplectic group $\mathrm{Sp}(4,\mathbb{R})$. Its Lie algebra $\mathfrak{sp}(4,\mathbb{R})$ has ten generators, which satisfy
%\begin{equation}
%X\in\mathfrak{sp}(4,\mathbb{R}):\quad X^TS+SX = 0\, ,
%\end{equation}
%where $S$ represents the symplectic product $\langle \cdot, \cdot \rangle $ on $\cH$ by $\langle v,w\rangle = v^T Sw$.
%In particular, all boundary operators, such as the $\slt$-triple, will be represented by $4\times 4$ matrices in $\mathfrak{sp}(4,\mathbb{R})$ or its complexification $\mathfrak{sp}(4,\mathbb{C})$. Note that in table \ref{table:data} we have chosen a different realization of $S$ for each type, simply for convenience.
%
%\begin{table}
%	\centering
%	\begin{tabular}{ | c | c | c | c |} \hline
%		operator &$\mathrm{I}_{1}$ & $\mathrm{II}_{0}$ & $\mathrm{IV}_{1}$ \\ \hline \hline
%		$N^+$ &  \rule[-1.05cm]{.0cm}{2.3cm} $\begin{pmatrix}
%		0 & 0 & 0 & 0 \\
%		0 & 0 & 1 & 0 \\
%		0 & 0 & 0 & 0 \\
%		0 & 0 & 0 & 0 \\
%		\end{pmatrix}$  & $\begin{pmatrix}
%		0 & 0 & 1 & 0 \\
%		0 & 0 & 0 & 1 \\
%		0 & 0 & 0 & 0 \\
%		0 & 0 & 0 & 0 \\
%		\end{pmatrix}$ & $\begin{pmatrix}
%		0 & 3 & 0 & 0 \\
%		0 & 0 & 2 & 0 \\
%		0 & 0 & 0 & 1 \\
%		0 & 0 & 0 & 0 \\
%		\end{pmatrix}$ \\ \hline
%		$N^0$ & \rule[-1.05cm]{.0cm}{2.3cm} $\begin{pmatrix}
%		0 & 0 & 0 & 0 \\
%		0 & 1 & 0 & 0 \\
%		0 & 0 & -1 & 0 \\
%		0 & 0 & 0 & 0 \\
%		\end{pmatrix}$ & $\begin{pmatrix}
%		1 & 0 & 0 & 0 \\
%		0 & 1 & 0 & 0 \\
%		0 & 0 & -1 & 0 \\
%		0 & 0 & 0 & -1 \\
%		\end{pmatrix}$ &  $\begin{pmatrix}
%		3 & 0 & 0 & 0 \\
%		0 & 1 & 0 & 0 \\
%		0 & 0 & -1 & 0 \\
%		0 & 0 & 0 & 3 \\
%		\end{pmatrix}$ \\ \hline
%		$N^-$ & \rule[-1.05cm]{.0cm}{2.3cm} $\begin{pmatrix}
%		0 & 0 & 0 & 0 \\
%		0 & 0 & 0 & 0 \\
%		0 & 1 & 0 & 0 \\
%		0 & 0 & 0 & 0 
%		\end{pmatrix}$  & $\begin{pmatrix}
%		0 & 0 & 0 & 0 \\
%		0 & 0 & 0 & 0 \\
%		1 & 0 & 0 & 0 \\
%		0 & 1 & 0 & 0 \\
%		\end{pmatrix}$ &   $\begin{pmatrix}
%		0 & 0 & 0 & 0 \\
%		1 & 0 & 0 & 0 \\
%		0 & 2 & 0 & 0 \\
%		0 & 0 & 3 & 0 
%		\end{pmatrix}$  \\ \hline
%		$Q_{\infty}$ &  \rule[-1.05cm]{.0cm}{2.3cm} $\begin{pmatrix}
%		0 & 0 & 0 & -\frac{3 i}{2} \\
%		0 & 0 & -\frac{i}{2} & 0 \\
%		0 & \frac{i}{2}  & 0 & 0 \\
%		\frac{3 i}{2} & 0 & 0 & 0 \\
%		\end{pmatrix}$ & $\begin{pmatrix}
%		0 & -i & -\frac{i}{2} & 0 \\
%		i & 0 & 0 & -\frac{i}{2} \\
%		\frac{i}{2} & 0 & 0 & -i \\
%		0 & \frac{i}{2} & i & 0 \\
%		\end{pmatrix}$ & $\begin{pmatrix}
%		0 & -\frac{3 i}{2} & 0 & 0 \\
%		\frac{i}{2} & 0 & -i & 0 \\
%		0 & i & 0 & -\frac{i}{2} \\
%		0 & 0 & \frac{3 i}{2} & 0 \\
%		\end{pmatrix}$ \\ \hline
%		$\delta$ & \rule[-1.05cm]{.0cm}{2.3cm}  $\begin{pmatrix}
%		0 & 0 & 0 & 0 \\
%		0 & 0 & 0 & 0 \\
%		0 & - c & 0 & 0 \\
%		0 & 0 & 0 & 0 
%		\end{pmatrix}$ & $\begin{pmatrix}
%		0 & 0 & 0 & 0 \\
%		0 & 0 & 0 & 0 \\
%		-c & 0 & 0 & 0 \\
%		0 & -c & 0 & 0 \\
%		\end{pmatrix}$ & $\begin{pmatrix}
%		0 & 0 & 0 & 0 \\
%		0 & 0 & 0 & 0 \\
%		0 & 0 & 0 & 0 \\
%		\chi & 0 & 0 & 0 
%		\end{pmatrix}$\\ \hline
%		$S$ & \rule[-1.05cm]{.0cm}{2.3cm}  $\begin{pmatrix} 0 & 0 & 0 & 1\\
%		0 & 0 & -1 & 0\\
%		0 & 1 & 0 & 0\\
%		-1 & 0 & 0 & 0 \end{pmatrix} $& $\begin{pmatrix}
%		0 & 0 & 1 & 0 \\
%		0 & 0 & 0 & 1 \\
%		-1 & 0 & 0 & 0 \\
%		0 & -1 & 0 & 0
%		\end{pmatrix}$ & $\begin{pmatrix}
%		0 & 0 & 0 & -1 \\
%		0 & 0 & 3 & 0 \\
%		0 & -3 & 0 & 0 \\
%		1 & 0 & 0 & 0 \\
%		\end{pmatrix}$ \\ \hline
%	\end{tabular}
%	\caption{\label{table:data} Characteristic data for the three possible kinds of boundaries of Calabi--Yau type with weight $3$ in two-dimensional (complex one-dimensional) moduli spaces. }
%\end{table}
%
%Let us now outline how the $\slt$-triples are constructed. The idea is to determine the irreducible $\slt$-representations fixed by the boundary type. Given this set of states, we can then simply write down generators that produce the corresponding spectrum. For the one-modulus boundaries we find
%\begin{equation}\label{eq:spectra}
%\begin{aligned}
%\mathrm{I}_{1} &: \qquad \left|0, 0 ; \tfrac{3}{2}\right\rangle\, , \ \  \left|1,1;\tfrac{1}{2}\right\rangle\, , \ \ \left|1,-1;-\tfrac{1}{2}\right\rangle\, , \ \ 
%\left|0, 0 ; -\tfrac{3}{2}\right\rangle \, , \\
%\mathrm{II}_{0} &: \qquad \left|1, 1 ; \tfrac{3}{2}\right\rangle\, , \ \  \left|1,-1;\tfrac{1}{2}\right\rangle\, , \ \  \left|1,1;-\tfrac{1}{2}\right\rangle\, , \ \ 
%\left|1, -1 ; -\tfrac{3}{2}\right\rangle \, , \\
%\mathrm{IV}_{1} &: \qquad \left|3, 3 ; \tfrac{3}{2}\right\rangle\, , \  \ \left|3,1;\tfrac{1}{2}\right\rangle\, , \  \ \left|3,-1;-\tfrac{1}{2}\right\rangle\, , \ \ 
%\left|3,-3 ; -\tfrac{3}{2}\right\rangle \, . \\
%\end{aligned}
%\end{equation}
%These spectra are obtained as follows. The presence of the states $|\hat{d},\hat{d};3/2\rangle$ and their descendants is given by \eqref{eq:principaltypes}. Under complex conjugation states $|d,s;q\rangle$ are mapped to $|d,-s;-q\rangle$, resulting in an additional set of states for $\mathrm{I}_{1}$ and $\mathrm{II}_{0}$ boundaries related to $|\hat{d},-\hat{d};-3/2\rangle$. For $\mathrm{II}_{0}$ and $\mathrm{IV}_{1}$ boundaries this information is already sufficient to fix their spectra. For $\mathrm{I}_{1}$ boundaries we infer from \eqref{eq:secondary_type} the presence of the states $|1,1;1/2\rangle$ and $|1,1;-1/2\rangle$ by the fact that $n=1$, which completes the spectrum. One can then take a simple form for the $\mathfrak{sl}(2,\mathbb{R})$-triple that has the right set of irreducible $\slt$-representations.  
%By switching to the $\mathfrak{sl}(2,\mathbb{C})$-triple via \eqref{eq:rho_switch} and matching the charges according to \eqref{eq:spectra} the generators $(L_{1},L_{0},L_{-1})$ and the charge operator $Q_{\infty}$ can then be constructed as well. 
%
%Finally we have to construct the phase operator $\delta$ for the boundaries, so let us briefly recall its properties. The operator $\delta$ needs to be a real map, an infinitesimal isometry of the symplectic pairing $S$ and commute with $N^{-}$. Furthermore, when we rotate to the complex basis by the transformation $\rho$ and expand into eigenoperators of $Q_{\infty}$ and $L_{0}$ it needs to have charge $1 \leq -q \leq 3$ and weight $1+q \leq -s \leq 4+q$. For $\mathrm{I}_{1}$ and $\mathrm{II}_{0}$ boundaries the only map that satisfies these criteria is the lowering operator $N^{-}$ itself, so the phase operator $\delta$ is fixed up to an overall proportionality constant $c$. For $\mathrm{IV}_{1}$ boundaries there are two independent maps, either $N^{-}$ or the map given for $\delta$ in table \ref{table:data}. For convenience we have set the component along $N^{-}$ to zero. This component simply amounts to a coordinate shift $y \to y-c$ for the bulk fields, as will be demonstrated by the bulk reconstruction for the $\mathrm{I}_{1}$ and $\mathrm{II}_{0}$ boundaries. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







\section{Conclusions}

%In this work we have studied the solutions of a special non-linear sigma-model depending on group-valued matter fields $h$
%varying over a two-dimensional space-time. This model was introduced to encode couplings 
%of certain supersymmetric effective field theories that are compatible with a UV completion in string theory. 
%In this application it is crucial to identify the two-dimensional space-time of the sigma-model
%with the moduli space of the effective theory.  
%Studying this sigma-model abstractly, i.e.~without any reference to the possibly underlying geometric string theory realization, we have 
%introduced a recursive way to reconstruct the matter field solutions near the boundaries of the two-dimensional space-time. 
%The reconstructed near-boundary solutions were uniquely fixed by a set of Sl(2)-boundary conditions 
%and a single matching condition. In applications to effective actions such solutions are of particular interest, since they encode couplings that are constrained by multiple swampland conjectures. Investigating these near-boundary solutions therefore provide us 
%with a general way to probe the string landscape in an abstract manner.
%Furthermore, the fact that the the solutions can be reconstructed starting from the boundary supports the holographic perspective put forward in 
%\cite{Grimm:2020cda} and gives an interesting realization of a bulk-boundary correspondence. 
%Notably, the proposed correspondence can be formulated independently of any geometric realization and is therefore intriguing in its own right. In this work we elucidated the abstract constructions that enter in this correspondence and successfully applied it to a particular set of examples. 
%
%
%In the reconstruction of the matter field solutions $h$ we restricted ourselves to solving 
%the equations of motion in a two-dimensional background metric that is flat up to a general Weyl factor.
%Furthermore, we imposed three conditions to control their asymptotic behaviour. First, we required the existence of a continuous symmetry 
%$h(x+c,y) = e^{cN^-} h(x,y)$ that arose as a continuous version of the discrete monodromy transformations. The universal emergence of such a continuous global symmetry at infinite distance boundaries in the associated effective theories is consistent with the recent discussions in  \cite{GPV,Lee:2019wij,Lanza:2020qmt}. The second restriction we imposed is the $Q$-constraint. We stress that this constraint does not follow from the action principle and should be regarded as an additional requirement to obtain `physical' solutions \cite{Cecotti:2020rjq,Grimm:2020cda}. It roughly states that 
%the solutions are compatible with the charge decomposition of the Hilbert space at every point near the boundary. 
%While mathematically well understood within asymptotic Hodge theory \cite{Schmid, CKS}, it would be interesting to give a 
%precise physical interpretation of this constraint from the point of view of the sigma-model. 
%In particular, it is desirable to check if it can be understood a gauge constraint in an extended version of the model. Lastly, we imposed specific boundary conditions on the matter fields. In particular, we demanded that the leading behaviour of the operators $\cN^\bullet(y)$, as $y\rightarrow\infty$, is governed by an $\slt$-triple. This triple plays a central role in the bulk reconstruction procedure through the boundary decomposition it induces on both the Hilbert space and the operators. Still, these three conditions do not fix the solution to the equations of motion completely. This is achieved by the matching condition with the phase operator $\delta$, which comprises the final piece of the boundary data. Indeed, while the $\slt$-triple specifies the leading behaviour of the matter fields, the CKS recursion together with the matching condition fixes all sub-leading terms $g_k$. 
%The striking result is that in this way a rather simple set of boundary conditions and the CKS recursion uniquely determines an infinite series of matrix-valued coefficients in the $1/y$-expansion. 
%
%In order to illustrate how the bulk reconstruction is performed in practice we have solved the CKS recursion for a concrete set of boundary data. From the classification of possible boundary data we have considered all examples that are of Calabi--Yau type in $D=3$ that 
%have $h_{1/2}=1$. The three possible cases were denoted by $\mathrm{I}_1$, $\mathrm{II}_0$ and $\mathrm{IV}_1$. 
%While it is important to stress that we did not require a geometric realization in order to arrive at this data, we have found that the corresponding 
%solutions  can be associated to three well-known degenerations realized in geometric Calabi--Yau threefold moduli spaces known as the conifold point, the 
%Tyurin degeneration, and the large complex structure point.  
%In order to make this identification we explained the relationship between the matter field solutions matching the sl(2) boundary data of Calabi--Yau type and the asymptotic period vector of the $(D,0)$-form on a Calabi--Yau $D$-fold. Here it is interesting to 
%note that the CKS recursions for the cases $\mathrm{I}_1$ and $\mathrm{II}_0$ admit rather simple solutions. Nevertheless we argued 
%that matching the bulk solutions to geometric periods one is able to determine that certain instanton corrections are 
%required in the asymptotic periods.
%In contrast, for the example $\mathrm{IV}_1$ the CKS recursion was much more involved and required solving a set of four coupled recursion relations, while its relation to the period vector is straightforward. The intricate dependence of the complexity of the procedure on the boundary data raises the question of whether it is possible to write down a general solution to the CKS recursion, especially when considering higher-dimensional moduli spaces, and poses an interesting challenge for future investigations. 
%
%
%
%There are numerous further avenues that can be taken to extend the proposed bulk-boundary correspondence and
%elucidate the physical nature of the model as a whole.
%As a first step we have already studied symmetries of the bulk action in this work. We discovered a global symmetry for left multiplication with an associated conserved current, while right multiplication gave rise to a gauge symmetry. In order to extend these models, one immediate question is to find a generalization to higher-dimensional moduli spaces. While the matter action admits a straightforward higher-dimensional generalisation  \cite{Cecotti:2020rjq}, it is very non-trivial to extend the holographic perspective and the CKS recursion.  To complement this, it is also interesting to couple the matter action to gravity. For the two dimensional settings considered here, we recall 
%that Einstein gravity is of topological nature. This fact, together with the desire to fix the background metric to be the so-called Weil-Petersson metric,  lead to the proposal of \cite{Grimm:2020cda} to couple the matter action to an alternative gravitational theory in two dimensions known as JT-gravity \cite{Teitelboim:1983ux,Jackiw:1984je}. In this proposal the Hodge metric, which is constructed from the on-shell conserved currents, is the crucial link between the matter action and the gravity action. While this proposal might be intriguing, it is also conceivable that the Hodge metric appears as the space-time metric itself. It is thus desirable to study the gravity coupled action in two dimensions and lay the groundwork for the generalization to higher dimensions. 
%
%Let us also briefly comment on the reconstruction of the period vector. Our discussion focussed on the derivation of the period vectors from 
%the bulk field solutions via the construction of a nilpotent orbit. We have then compared these results with the known leading 
%expressions for the period vector for Calabi--Yau threefold examples. In an upcoming project, it is shown how bulk solutions with sl(2) boundary data can always be integrated to an asymptotic period vector \cite{Bastiantoappear}. This yields the immediate question of whether or not one can reconstruct the full period vector on the entire moduli space including all instanton corrections when taking into account the data supplied for all boundaries. This would imply the exciting possibility that in fact the full bulk geometry is entirely encoded in the boundary information and would give further support for the existence 
%of a fully holographic description of the moduli space. 
%
%
%In developing further a holographic perspective one also has to face several open questions regarding the boundary information. The first is whether there exists a proper `boundary theory' that may give rise to the various components of the boundary data in a physical manner. Note that both the Hodge metric and the Weil-Petersson metric, the latter at infinite distance boundaries, asymptote to an $\mathrm{AdS}_2$ metric. This  indicates that 
%the encountered bulk-boundary correspondence is some manifestation of the $\mathrm{AdS}_2$/$\mathrm{CFT}_1$ duality. 
%Especially interesting in this regard is the role that the phase operator would play in such a boundary theory. Indeed, the origin of the phase operator, as well as the matching condition are crucial in order to understand the bulk-boundary correspondence further, and it is tempting to speculate that the proposed presence of emergent and axionic strings \cite{Lee:2018urn,Lee:2018spm,Marchesano:2019ifh,Lee:2019xtm,Lee:2019wij, Baume:2019sry, Lanza:2020qmt,Klaewer:2020lfg, Lanzatoappear} could serve 
%as a guide to clarify their appearance. It is important to emphasize that while we have restricted our discussion of explicit examples to boundaries of Calabi--Yau type this was purely a choice made to connect with the existing swampland literature. In elucidating the bulk-boundary correspondence it would be illustrative to reconstruct the bulk solutions for boundaries that are not of Calabi--Yau type. For example it is interesting to consider the moduli spaces of Riemann surfaces, since these are already well-studied from the Hodge theory perspective \cite{Hain:2003}. It is an exciting prospect that already by changing the boundary conditions the holographic approach may also be extended to certain non-supersymmetric effective actions. 




